A Set-Theoretic Study of the Relationships of Image Models and Priors for Restoration Problems

Image prior modeling is the key issue in image recovery, computational imaging, compresses sensing, and other inverse problems. Recent algorithms combining multiple effective priors such as the sparse or low-rank models, have demonstrated superior performance in various applications. However, the relationships among the popular image models are unclear, and no theory in general is available to demonstrate their connections. In this paper, we present a theoretical analysis on the image models, to bridge the gap between applications and image prior understanding, including sparsity, group-wise sparsity, joint sparsity, and low-rankness, etc. We systematically study how effective each image model is for image restoration. Furthermore, we relate the denoising performance improvement by combining multiple models, to the image model relationships. Extensive experiments are conducted to compare the denoising results which are consistent with our analysis. On top of the model-based methods, we quantitatively demonstrate the image properties that are inexplicitly exploited by deep learning method, of which can further boost the denoising performance by combining with its complementary image models.

==> exp_denoising.tex <==
\section{Image Denoising Experiments} \label{sec idk}


\begin{table}[h!]
\centering
\begin{tabular}{||r c c c c||} 
 \hline
 & $\sigma$ =5  & $\sigma$ =10  & $\sigma$ =15  & $\sigma$ =25 \\
 \hline\hline
OCTOBOS  & 38.27  & 34.24  & 32.16  & 29.60 \\
SAIST  & 38.39  & 34.51  & 32.39  & 29.93 \\
OCTOBOS + SAIST  & 38.50  & 34.59  & 32.50  & 30.02 \\
$\Delta$ Average PSNR mean& 0.10  & 0.08  & 0.11  & 0.09 \\
$\Delta$ Average PSNR std & 0.03  & 0.03  & 0.04  & 0.04 \\
 \hline
\end{tabular}
\caption{Average PSNR of denoised Kodak set by OCTOBOS, SAIST, their combination and improved PSNR (mean and std) under different noise levels}
\label{table:im_denoise_1}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{||r c c c c||} 
 \hline
 & $\sigma$ =5  & $\sigma$ =10  & $\sigma$ =15  & $\sigma$ =25 \\
 \hline\hline
KSVD  & 37.60  & 33.70  & 31.59  & 29.12 \\
OCTOBOS  & 38.27  & 34.24  & 32.16  & 29.60 \\
KSVD + OCTOBOS  & 38.28  & 34.30  & 32.20  & 29.64 \\
$\Delta$ Average PSNR mean& 0.01  & 0.07  & 0.04  & 0.04 \\
$\Delta$ Average PSNR std & 0.01  & 0.03  & 0.02  & 0.02 \\
 \hline
\end{tabular}
\caption{Average PSNR of denoised Kodak set by KSVD, OCTOBOS, their combination and improved PSNR (mean and std) under different noise levels}
\label{table:im_denoise_2}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{||r c c c c||} 
 \hline
 & $\sigma$ =5  & $\sigma$ =10  & $\sigma$ =15  & $\sigma$ =25 \\
 \hline\hline
GSM  & 38.37  & 34.48  & 32.37  & 29.76 \\
OCTOBOS  & 38.27  & 34.24  & 32.16  & 29.60 \\
GSM + OCTOBOS  & 38.50  & 34.58  & 32.53  & 29.97 \\
$\Delta$ Average PSNR mean& 0.12  & 0.10  & 0.14  & 0.15 \\
$\Delta$ Average PSNR std & 0.04  & 0.04  & 0.05  & 0.05 \\
 \hline
\end{tabular}
\caption{Average PSNR of denoised Kodak set by GSM, OCTOBOS, their combination and improved PSNR (mean and std) under different noise levels}
\label{table:im_denoise_3}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{||r c c c c||} 
 \hline
 & $\sigma$ =5  & $\sigma$ =10  & $\sigma$ =15  & $\sigma$ =25 \\
 \hline\hline
GSM  & 38.37  & 34.48  & 32.37  & 29.76 \\
SAIST  & 38.39  & 34.51  & 32.39  & 29.93 \\
GSM + SAIST  & 38.46  & 34.60  & 32.49  & 29.99 \\
$\Delta$ Average PSNR & 0.06  & 0.07  & 0.07  & 0.05 \\
$\Delta$ Average PSNR std & 0.02  & 0.02  & 0.03  & 0.04 \\
 \hline
\end{tabular}
\caption{Average PSNR of denoised Kodak set by GSM, SAIST, their combination and improved PSNR (mean and std) under different noise levels}
\label{table:im_denoise_4}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{||r c c c c||} 
 \hline
 & $\sigma$ =15  & $\sigma$ =25  & $\sigma$ =50  & $\Delta $ PSNR\\
 \hline\hline
DnCNN  & 32.89  & 30.47  & 27.49 & 0.00\\
DnCNN + KSVD  & 32.89  & 30.47  & 27.49 & 0.00\\
DnCNN + GSM  & 32.94  & 30.52  & 27.58 & 0.06\\
DnCNN + WNNM  & 32.95  & 30.55  & 27.60 & 0.08\\ 
\hline
\end{tabular}
\caption{Average PSNR of denoised Kodak set by DnCNN, its combination with other methods, and improved PSNR (mean)}
\label{table:im_denoise_5}
\end{table}


% \begin{table}[h!]
% \centering
% \begin{tabular}{||r c c c c||} 
%  \hline
%  & $\sigma$ =30  & $\sigma$ =50  & $\sigma$ =70  & $\Delta $ PSNR\\
%  \hline\hline
% DnCNN  & 27.04  & 24.40  & 22.61 & 0.00\\
% DnCNN + WNNM  & 27.77  & 25.06  & 23.34 & 0.71\\
% \hline
% \end{tabular}
% \caption{Average PSNR of denoised Urban 100 LR images by DnCNN, its combination with other methods, and improved PSNR (mean)}
% \label{table:im_denoise_6}
% \end{table}


\begin{table}[h!]
\centering
\begin{tabular}{||r c c c c||} 
 \hline
 & $\sigma$ =30  & $\sigma$ =50  & $\sigma$ =70  & $\Delta $ PSNR\\
 \hline\hline
DnCNN  & 28.16  & 25.48  & 23.61 & 0.00\\
DnCNN + KSVD  & 28.21  & 25.52  & 23.64 & 0.04\\
DnCNN + GSM  & 28.74  & 26.07  & 24.33 & 0.63\\
DnCNN + WNNM  & 28.99  & 26.25  & 24.47 & 0.82\\
DnCNN + GSM + WNNM & 28.99  & 26.26  & 24.50 & 0.84\\
DnCNN + KSVD + GSM & 28.74  & 26.07  & 24.33 & 0.63\\
DnCNN + KSVD + WNNM & 28.99  & 26.25  & 24.47 & 0.82\\
\hline
\end{tabular}
\caption{Average PSNR of denoised Urban 100 SF2 images by DnCNN, its combination with other methods ($\lambda$ is the best given the ground truth), and improved PSNR (mean)}
\label{table:im_denoise_7}
\end{table}

% \begin{table}[h!]
% \centering
% \begin{tabular}{||r c c c c||} 
%  \hline
%  & $\sigma$ =30  & $\sigma$ =50  & $\sigma$ =70  & $\Delta $ PSNR\\
%  \hline\hline
% DnCNN  & 27.04  & 24.40  & 22.61 & 0.00\\
% DnCNN + WNNM  & 27.62  & 24.92  & 23.16 & 0.55\\
% \hline
% \end{tabular}
% \caption{Average PSNR of denoised Urban 100 LR images by DnCNN, its combination with other methods ($\lambda=0.5$), and improved PSNR (mean)}
% \label{table:im_denoise_8}
% \end{table}


\begin{table}[h!]
\centering
\begin{tabular}{||r c c c c||} 
 \hline
 & $\sigma$ =30  & $\sigma$ =50  & $\sigma$ =70  & $\Delta $ PSNR\\
 \hline\hline
DnCNN  & 28.16  & 25.48  & 23.61 & 0.00\\
DnCNN + KSVD  & 27.94  & 25.20  & 23.26 & -0.29\\
DnCNN + GSM  & 28.64  & 25.97  & 24.17 & 0.51\\
DnCNN + WNNM  & 28.82  & 26.09  & 24.26 & 0.64\\
\hline
\end{tabular}
\caption{Average PSNR of denoised Urban 100 SF2 images by DnCNN, its combination with other methods ($\lambda=0.5$), and improved PSNR (mean)}
\label{table:im_denoise_9}
\end{table}


NOTE HERE:\\
When combining two methods at a given noise level, we traversed the $\mu \in {0:0.1:1}$ and found the best combination based on 10 randomly chosen image from urban100 dataset. The average of $\mu$ was then fixed and applied to the rest of the 90 images.  

\begin{table}[h!]
\centering
\begin{tabular}{||r c c c c||} 
 \hline
 & $\sigma$ =30  & $\sigma$ =50  & $\sigma$ =70  & $\Delta $ PSNR\\
 \hline\hline
DnCNN  & 28.16  & 25.48  & 23.61 & 0.00\\
DnCNN + KSVD  & 28.11  & 25.52  & 23.64 & 0.01\\
DnCNN + GSM  & 28.69  & 25.92  & 24.11 & 0.49\\
DnCNN + WNNM  & 28.95  & 26.05  & 24.39 & 0.71\\
\hline
\end{tabular}
\caption{Average PSNR of denoised Urban 100 SF2 images by DnCNN, its combination with other methods ($\lambda$ tuned), and improved PSNR (mean)}
\label{table:im_denoise_10}
\end{table}

%%%%%%%%%%%%% back up %%%%%%%%%%% mu = 0.5 result


%%%%%%%%%%%%%%%%%%%%%%%% DnCNN in Urban100 %%%%%%%%%%%%%%%%%%%%%
\begin{table}[h!]
\centering
\fontsize{9}{14pt}\selectfont
\begin{tabular}{|| r | c c c | c||} 
 \hline
 & $\sigma$ =30  & $\sigma$ =50  & $\sigma$ =70  & $\Delta $ PSNR\\
 \hline\hline
DnCNN  & 28.16  & 25.48  & 23.61 & 0.00\\
DnCNN + KSVD  & 27.94  & 25.20  & 23.26 & -0.29\\
DnCNN + SSC-GSM  & 28.64  & 25.97  & 24.17 & 0.51\\
DnCNN + WNNM  & \textbf{28.82}  & \textbf{26.09}  & \textbf{24.26} & \textbf{0.64}\\
\hline
\end{tabular}
\caption{Average PSNR of the denoised images from the Urban100 Dataset \cite{huang2015single} by DnCNN, and its combination with KSVD, SSC-GSM, and WNNM, with their corresponding improved PSNRs. The highest PSNRs for each $sigma$ and the highest $\Delta$ PSNR are highlighted in bold.}
\label{table:im_denoise_5}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
